Leveraging Multimodal Features and Item-level User Feedback for Bundle Construction

Automatic bundle construction is a crucial prerequisite step in various bundle-aware online services. Previous approaches are mostly designed to model the bundling strategy of existing bundles. However, it is hard to acquire large-scale well-curated bundle dataset, especially for those platforms that have not offered bundle services before. Even for platforms with mature bundle services, there are still many items that are included in few or even zero bundles, which give rise to sparsity and cold-start challenges in the bundle construction models. To tackle these issues, we target at leveraging multimodal features, item-level user feedback signals, and the bundle composition information, to achieve a comprehensive formulation of bundle construction. Nevertheless, such formulation poses two new technical challenges: 1) how to learn effective representations by optimally unifying multiple features, and 2) how to address the problems of modality missing, noise, and sparsity problems induced by the incomplete query bundles. In this work, to address these technical challenges, we propose a Contrastive Learning-enhanced Hierarchical Encoder method (CLHE). Specifically, we use self-attention modules to combine the multimodal and multi-item features, and then leverage both item- and bundle-level contrastive learning to enhance the representation learning, thus to counter the modality missing, noise, and sparsity problems. Extensive experiments on four datasets in two application domains demonstrate that our method outperforms a list of SOTA methods. The code and dataset are available at https://github.com/Xiaohao-Liu/CLHE.

==> 1_introduction_old.tex <==
\section{Introduction} \label{sec:introduction}

Product bundling has been a practical and effective marketing strategy, tracing back from the ancient commercial times and persisting through to nowadays rapidly growing e-commerce and online services. By combining a set of individual items into a bundle, both sellers (or service providers) and consumers can benefit a lot from multiple aspects, such as reducing cost of packaging, shipment, and installation, \etc or promoting sales by applying discounts. To implement product bundling, the first and foremost step is constructing bundles from individual items, \aka bundle construction, which is conventionally conducted by human experts. However, the explosive growth of item set poses significant challenges to such high cost manual approaches, therefore, automatic solutions for bundle construction are imperative and have garnered more and more attention in recent years.   

Previous efforts on automatic bundle construction can be sorted into two strands based on the input information: bundle-item affiliation and item content information. First, the bundle-item affiliations elicit the item-item co-occurrence information, preserving the relations among items that could explain why such items can be put together. For example, the items are compatible in terms of functions or with similar styles. Second, the item content information, such as texts, images, audio, or metadata, is complementary to the bundle-item affiliation information, aiming to enhance the representation expressiveness especially for long-tail and cold-start items. Even though various methods have been developed using these two types of data, we argue that the user-item interactions, which are well studied in personalized recommendation tasks, however, are less explored in the bundle construction problem. 

We argue that, in the task of bundle construction, user-item interaction is the third type of information that is of large amount, easy to access, while offering irreplaceable information against the previous two types of data. Intuitively, the items that users frequently co-interact with are more likely to be included in a bundle. This is because the signals reflected by user behaviors are post-hoc observations that could not be perfectly foreseen beforehand. Therefore, in contrast to the prior knowledge from existing bundle compositions, the users' implicit feedback provides precious crowd-sourcing knowledge, which is more diverse catering to real world scenarios. More importantly, new items are continuously pushed online, however, these cold-start items have not been included in any bundle before and can only be served individually. In such cases, a few user-item interactions would be the minimal accessible information, which is weak while especially precious to guide the bundle construction. To be noted, the user-item interactions are not necessarily collected from the same platform that hosts the bundle service. For example, user feedback collected from last.fm can be used by Spotify to consturct music playlist, only if there are shared items across platforms. Consequently, the difficulty of data collection is significantly alleviated.

Based on the aforementioned motivation, we aim to leverage the rich user-item interactions, along with the existing bundle-item affiliation and item content information, to achieve a comprehensive formulation of multimodal bundle construction. However, it is non-trivial to model all the three types of information and achieve optimal bundle construction performance. First, how to well capture the cooperative association among the three modalities, to maximize the complementary effects while minimize the conflicting effects, is a key challenge. Second, only a small portion of items have rich interactions for both bundle-item affiliations and user-item interactions, and the cold-start problem in certain modalities poses exceptional challenge. 

In this work, to address the aforementioned challenges, we propose a \textbf{H}ierarchical \textbf{C}ontrastive \textbf{E}ncoder for \textbf{M}utimodal \textbf{B}undle \textbf{C}onstruction, short as \textbf{HCE4MBC}. Specifically, we pre-train a collaborative filtering (CF)-based model to retain the user-item information. We take advantage of the recently proposed large-scale multimodal foundation model to extract the content features of items. Then, we employ a hierarchical encoder to obatin the query bundle representation, where two self-attention layers are leveraged to fuse multimodal information and multiple item representations. To tackle the cold-start problem, we take advantage the contrastive learning to mine the self-supervised signals. Particularly, we apply two level of contrastive losses to item and bundle representations, respectively. We conduct experiments on two domains, \ie music playlist and fashion outfit, each of which has two versions of datasets with different sparsity. Experimental results demonstrate that our method outperforms state-of-the-art (SOTA) methods by a large margin. Various ablation and modal studies further justify the key modules of our methods and demystify the working mechanism of our proposed model. We summarize the key contributions of this work as follows:

\begin{itemize}[leftmargin=*]
    \item To the best of our knowledge, we are the first to systematically analyze the role of user feedback in multimodal bundle construction and propose a more comprehensive formulation of multimodal bundle construction. 
    \item We propose a novel method of hiearchical contrastive transformer to solve the problem.
    \item Our method outperforms SOTA methods by a large margin on four datasets from two application domains. 
\end{itemize}

%\begin{figure}
%    \centering
%    \includegraphics[width = 0.95\linewidth]{figures/motivation.pdf}
%    %\vspace{-5pt}
%    \caption{The main motivation of context-aware event forecasting. (a) Most current events fall in the coarse-grained and higher level types of the ontology, while more informative fine-grained events are fewer. (b) Out-of-ontology and diverse contexts affect events. Context can provide more fine-grained information and enhance the event forecasting performance.}
%    \label{fig:motivation}
%    \vspace{-15pt}
%\end{figure}

==> 6_ethics_statement.tex <==
\section*{Ethics Statement}
In conducting this research, we have utilized datasets derived from publicly available sources. All user-specific information within these datasets has been anonymized to prevent potential breaches of privacy. Rights pertaining to the features of the items, encompassing text, images, and audio, remain the sole property of the original rights holders. This study is intended exclusively for academic purposes. Any subsequent implementation of the proposed algorithm in a production environment is at the discretion of the user, who should acknowledge and assume responsibility for any potential economic or societal implications.
